AI as a Medical Ally: Evaluating ChatGPT's Usage and Impact in Indian Healthcare

This study investigates the integration and impact of Large Language Models (LLMs), like ChatGPT, in India's healthcare sector. Our research employs a dual approach, engaging both general users and medical professionals through surveys and interviews respectively. Our findings reveal that healthcare professionals value ChatGPT in medical education and preliminary clinical settings, but exercise caution due to concerns about reliability, privacy, and the need for cross-verification with medical references. General users show a preference for AI interactions in healthcare, but concerns regarding accuracy and trust persist. The study underscores the need for these technologies to complement, not replace, human medical expertise, highlighting the importance of developing LLMs in collaboration with healthcare providers. This paper enhances the understanding of LLMs in healthcare, detailing current usage, user trust, and improvement areas. Our insights inform future research and development, underscoring the need for ethically compliant, user-focused LLM advancements that address healthcare-specific challenges.

==> files/061-acknowledgements.tex <==
We express our gratitude to the anonymous reviewers for their invaluable feedback, which significantly enhanced the overall quality of the paper. Additionally, we extend our thanks to Shamik Sinha, Palak Bhardwaj, Rayyan Hussain, Kashvi Panvanda, Sidhartha Garg, Shagun Yadav, Yash Chillar, and Sourav Goyal for their assistance in the development of survey and interview questionnaires, as well as their involvement in conducting selected interviews.
